A Survey of Methods for Collective Communication Optimization and Tuning

New developments in HPC technology in terms of increasing computing power on multi/many core processors, high-bandwidth memory/IO subsystems and communication interconnects, pose a direct impact on software and runtime system development. These advancements have become useful in producing high-performance collective communication interfaces that integrate efficiently on a wide variety of platforms and environments. However, number of optimization options that shows up with each new technology or software framework has resulted in a \emph{combinatorial explosion} in feature space for tuning collective parameters such that finding the optimal set has become a nearly impossible task. Applicability of algorithmic choices available for optimizing collective communication depends largely on the scalability requirement for a particular usecase. This problem can be further exasperated by any requirement to run collective problems at very large scales such as in the case of exascale computing, at which impractical tuning by brute force may require many months of resources. Therefore application of statistical, data mining and artificial Intelligence or more general hybrid learning models seems essential in many collectives parameter optimization problems. We hope to explore current and the cutting edge of collective communication optimization and tuning methods and culminate with possible future directions towards this problem.

==> Makefile <==
NAME=collectives-tuning

GRAPHS=
FILES=abstract.tex section_1.tex section_2.tex section_3.tex section_4.tex sigproc.bib

all: ${NAME}.pdf

${NAME}.pdf: ${NAME}.tex ${FILES} ${GRAPHS}
	latexmk -bibtex-cond -shell-escape -pdf ${NAME}

clean:
	latexmk -C ${NAME}
	rm ${NAME}.bbl

realclean: clean
	rm -f *~

strip:
	for i in ${FILES}; \
	do grep -v "^[\\%][a-zA-Z ].*" ${i} > ${i}.stripped; \
	done 

count: strip
	wc -w *.stripped


